Inclusive-PIM: Hardware-Software Co-design for Broad Acceleration on Commercial PIM Architectures

Continual demand for memory bandwidth has made it worthwhile for memory vendors to reassess processing in memory (PIM), which enables higher bandwidth by placing compute units in/near-memory. As such, memory vendors have recently proposed commercially viable PIM designs. However, these proposals are largely driven by the needs of (a narrow set of) machine learning (ML) primitives. While such proposals are reasonable given the the growing importance of ML, as memory is a pervasive component, %in this work, we make there is a case for a more inclusive PIM design that can accelerate primitives across domains. In this work, we ascertain the capabilities of commercial PIM proposals to accelerate various primitives across domains. We first begin with outlining a set of characteristics, termed PIM-amenability-test, which aid in assessing if a given primitive is likely to be accelerated by PIM. Next, we apply this test to primitives under study to ascertain efficient data-placement and orchestration to map the primitives to underlying PIM architecture. We observe here that, even though primitives under study are largely PIM-amenable, existing commercial PIM proposals do not realize their performance potential for these primitives. To address this, we identify bottlenecks that arise in PIM execution and propose hardware and software optimizations which stand to broaden the acceleration reach of commercial PIM designs (improving average PIM speedups from 1.12x to 2.49x relative to a GPU baseline). Overall, while we believe emerging commercial PIM proposals add a necessary and complementary design point in the application acceleration space, hardware-software co-design is necessary to deliver their benefits broadly.

==> imperfect_workloads.tex <==
\section{Imperfect PIM Amenability}

% app, mem-limited, operand locality, no data reuse, aligned data parallelism, low register pressure
\begin{table*}
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c| } 
\hline
Application & Memory-limited & Operand locality & No data reuse & Aligned data parallelism & Low register pressure \\
\hline
Graph analytics & \checkmark & \checkmark & & & \checkmark \\ 
Wavesim & \checkmark & \checkmark & \checkmark & \checkmark &  \\ 
Sparse skinny GEMM & \checkmark & \checkmark & & & \checkmark \\ 
\hline
\end{tabular}
\end{center}
\end{table*}

\begin{itemize}
    \item Graph analytics: 
    \item Wavesim:
    \item Sparse skinny GEMM: 
\end{itemize}

\subsection{Workload overview and PIM limitation}

Graph nodes are processed in parallel, which involves updating nodes based on connected node values. For most realistic graphs, these workloads are often limited by memory throughput. However, there can be significant cache reuse depending on connectivity.

Limited by data reuse: Updates to highly connected nodes can exhibit high cache reuse - preventing this by flushing all data to memory can significantly harm performance.

Target data not aligned: Updates generated from a single node are unlikely to be aligned in different banks in the same channel, preventing the use of broadcast operations.

